Exploiting Distribution Constraints for Scalable and Efficient Image Retrieval

Image retrieval is crucial in robotics and computer vision, with downstream applications in robot place recognition and vision-based product recommendations. Modern retrieval systems face two key challenges: scalability and efficiency. State-of-the-art image retrieval systems train specific neural networks for each dataset, an approach that lacks scalability. Furthermore, since retrieval speed is directly proportional to embedding size, existing systems that use large embeddings lack efficiency. To tackle scalability, recent works propose using off-the-shelf foundation models. However, these models, though applicable across datasets, fall short in achieving performance comparable to that of dataset-specific models. Our key observation is that, while foundation models capture necessary subtleties for effective retrieval, the underlying distribution of their embedding space can negatively impact cosine similarity searches. We introduce Autoencoders with Strong Variance Constraints (AE-SVC), which, when used for projection, significantly improves the performance of foundation models. We provide an in-depth theoretical analysis of AE-SVC. Addressing efficiency, we introduce Single-shot Similarity Space Distillation ((SS)$_2$D), a novel approach to learn embeddings with adaptive sizes that offers a better trade-off between size and performance. We conducted extensive experiments on four retrieval datasets, including Stanford Online Products (SoP) and Pittsburgh30k, using four different off-the-shelf foundation models, including DinoV2 and CLIP. AE-SVC demonstrates up to a $16\%$ improvement in retrieval performance, while (SS)$_2$D shows a further $10\%$ improvement for smaller embedding sizes.

==> figure_tex/ablation_pca.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.75\textwidth]{figs/theory_pca_ablations.png}
  \caption{\small\textbf{Ablation study of standardization and dimension selection.} \spacename\ (orange) notably enhances performance on both datasets. \spacename\ is significantly better than standardization (pink) indicating that projecting image embeddings into an orthogonal space (PCA) before standardization is crucial, aligning with our theoretical analysis. Moreover, even post-PCA projection and standardization, dimensions with higher eigenvalues tend to be more important for retrieval as reflected in the difference between \spacename(orange) and VA-PCA-RS (brown).}
  \label{fig:theory_pca_ablations}
  \vspace{-1.5em}
\end{figure}


==> figure_tex/teaser.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/teaser.png} % Replace with your figure file
    \caption{Caption for the figure}
    \label{fig:teaser}
\end{wrapfigure}

